LiDAR-BEVMTN: Real-Time LiDAR Bird's-Eye View Multi-Task Perception Network for Autonomous Driving

LiDAR is crucial for robust 3D scene perception in autonomous driving. LiDAR perception has the largest body of literature after camera perception. However, multi-task learning across tasks like detection, segmentation, and motion estimation using LiDAR remains relatively unexplored, especially on automotive-grade embedded platforms. We present a real-time multi-task convolutional neural network for LiDAR-based object detection, semantics, and motion segmentation. The unified architecture comprises a shared encoder and task-specific decoders, enabling joint representation learning. We propose a novel Semantic Weighting and Guidance (SWAG) module to transfer semantic features for improved object detection selectively. Our heterogeneous training scheme combines diverse datasets and exploits complementary cues between tasks. The work provides the first embedded implementation unifying these key perception tasks from LiDAR point clouds achieving 3ms latency on the embedded NVIDIA Xavier platform. We achieve state-of-the-art results for two tasks, semantic and motion segmentation, and close to state-of-the-art performance for 3D object detection. By maximizing hardware efficiency and leveraging multi-task synergies, our method delivers an accurate and efficient solution tailored for real-world automated driving deployment. Qualitative results can be seen at https://youtu.be/H-hWRzv2lIY.

==> results/table-data-aug.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Comparison between static data augmentations (all augmentation applied in every epoch) vs progressive data augmentation (task specific augmentations applied in late stages of training).}
\label{tab:data-aug-static-progressive}
\begin{tabular}{@{}c|lllllll|l@{}}
\toprule
\multirow{2}{*}{Augmentation} & \multicolumn{3}{c|}{Object Detection} & \multicolumn{4}{c|}{Semantic Segmentation} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Motion\\ Seg.\end{tabular}}} \\ \cmidrule(lr){2-8}
 & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Moderate} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Car} & \multicolumn{1}{c}{Road} & \multicolumn{1}{c}{Building} & \multicolumn{1}{c|}{Veg.} & \multicolumn{1}{c}{} \\ \midrule
Static aug. & 96.27 & 94.20 & 89.10 & 93.00 & 95.32 & 84.35 & 81.10 & 68.16 \\
Progressive aug. & \textbf{96.34} & 94.00 & \textbf{90.01} & \textbf{96.18} & \textbf{96.12} & \textbf{84.50} & 81.09 & \textbf{73.14} \\ \bottomrule
\end{tabular}
\end{table}

==> results/table6-LAT.tex <==
\begin{table}[t]
\centering
\captionsetup{singlelinecheck=false, font=small, skip=2pt, belowskip=-2pt}
\caption{\textbf{Inference latency comparison}- MTL and STL networks for object detection, semantic segmentation, and motion segmentation. MTL - 3 tasks achieves 2x speed up over three single task networks.}
\label{tab:table-latency-comparison}
\begin{adjustbox}{width=\columnwidth}
\setlength{\tabcolsep}{0.2em}
\begin{tabular}{@{}l|ccc|c@{}}
\toprule
\multicolumn{1}{c|}{} & 
\multicolumn{3}{c|}{FP16 inference latency (ms)} & \\ 
\cmidrule(lr){2-4}
\multicolumn{1}{c|}{\multirow{-2}{*}{Task combination}} &
  \cellcolor[HTML]{FFCCC9}\textit{Encoder} &
  \cellcolor[HTML]{FFFFC7}\textit{\begin{tabular}[c]{@{}c@{}}Decoder+\\ Heads\end{tabular}} &
  \cellcolor[HTML]{ECF4FF}\textit{Total} &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Speedup\\ factor\end{tabular}} \\ \midrule
STL(OD) + STL(SS) + STL(MS) & \multicolumn{1}{c|}{8.80}          & \multicolumn{1}{c|}{4.00}          & 12.80          & baseline      \\
STL (OD) + MTL(SS + MS)     & \multicolumn{1}{c|}{6.10}          & \multicolumn{1}{c|}{2.55}          & 8.65          & 1.47          \\
STL(MS) + MTL(OD + SS)      & \multicolumn{1}{c|}{6.10}          & \multicolumn{1}{c|}{2.73}          & 8.83          & 1.44          \\
\textbf{MTL (OD + SS + MS)} & \multicolumn{1}{c|}{\textbf{4.30}} & \multicolumn{1}{c|}{\textbf{1.71}} & \textbf{6.01} & \textbf{2.12} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


\begin{table}[t]
\centering
\captionsetup{singlelinecheck=false, font=small, skip=2pt, belowskip=-2pt}
\caption{\textbf{Comparison between static data augmentations vs progressive data augmentation.}}
\label{tab:data-aug-static-progressive}
\begin{adjustbox}{width=\columnwidth}
\setlength{\tabcolsep}{0.2em}
\begin{tabular}{@{}l|lllllll|l@{}}
\toprule
 & \multicolumn{3}{c|}{Object Detection} & \multicolumn{4}{c|}{Semantic Segmentation} & \multicolumn{1}{c}{} \\ \cmidrule(lr){2-8}
\multirow{-2}{*}{Augmentation} & \multicolumn{1}{c}{\cellcolor[HTML]{9AFF99}Easy} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFC7}Mod.} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCCC9}Hard} & \multicolumn{1}{c}{\cellcolor[HTML]{96FFFB}Car} & \multicolumn{1}{c}{\cellcolor[HTML]{FFCCC9}Road} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}Build.} & \multicolumn{1}{c|}{\cellcolor[HTML]{32CB00}Veg.} & \multicolumn{1}{c}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Motion\\ Seg.\end{tabular}}} \\ \midrule
Static aug. & 96.27 & 94.20 & 89.10 & 93.00 & 95.32 & 84.35 & 81.10 & 68.16 \\
\textbf{Progressive aug.} & \textbf{96.34} & 94.00 & \textbf{90.01} & \textbf{96.18} & \textbf{96.12} & \textbf{84.50} & 81.09 & \textbf{73.14} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


% ---------------------------------------------------------------------------------------------------------------%


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t!]
\centering
\captionsetup{singlelinecheck=false, font=small, skip=2pt, belowskip=-2pt}
\caption{\textbf{Runtime analysis of encoder and decoder building blocks
under different optimization conditions in a single task context:} \textcolor{blue}{vanilla pytorch (pth), pruning with maximum 50\% sparsity (prune), conversion to tensorrt FP16 (trt16), pruning followed by conversion to tensorrt FP16 (prune + trt16)}}
\label{tab:timing-details}
\scalebox{0.99}{
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}c|cccccccc@{}}
\toprule
 & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Downsampling Blocks\\ (Encoder)\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}Upsampling Blocks\\ (Decoder)\end{tabular}} \\ \cmidrule(l){2-9} 
\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Block\\ index\end{tabular}} & \cellcolor[HTML]{FFCCC9}\textit{\textbf{pth}} & \cellcolor[HTML]{FFCE93}\textit{\textbf{prune}} & \cellcolor[HTML]{FFFC9E}\textit{\textbf{trt16}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textit{\textbf{\begin{tabular}[c]{@{}c@{}}prune +\\ trt16\end{tabular}}}} & \cellcolor[HTML]{FFCCC9}\textit{\textbf{pth}} & \cellcolor[HTML]{FFCE93}\textit{\textbf{prune}} & \cellcolor[HTML]{FFFC9E}\textit{\textbf{trt16}} & \cellcolor[HTML]{9AFF99}\textit{\textbf{\begin{tabular}[c]{@{}c@{}}prune +\\ trt16\end{tabular}}} \\ \midrule
1 & 20.99 & 12.10 & 4.11 & 2.12 & 11.20 & 8.10 & 2.16 & 1.02 \\
2 & 11.81 & 8.03 & 2.12 & 1.48 & 7.69 & 5.11 & 1.00 & 0.40 \\
3 & 7.98 & 4.45 & 1.20 & 1.30 & 6.11 & 4.71 & 0.56 & 0.30 \\
4 & 6.98 & 3.01 & 1.10 & 1.05 & 5.57 & 3.96 & 0.61 & 0.23 \\
5 & 6.19 & 3.01 & 1.10 & 1.01 & 5.07 & 2.96 & 0.50 & 0.12 \\
\rowcolor[HTML]{EFEFEF} 
\textit{Total} & 53.95 & 30.60 & 9.63 & \textbf{6.96} & 35.64 & 24.84 & 4.83 & \textbf{2.07} \\ \bottomrule
\end{tabular}
\end{adjustbox}
}
\end{table}


\begin{table*}[htb!]
\caption{\textbf{Evaluation on Waymo validation set:} \textcolor{blue}{Comparision of 3D object detection and semantic segmentation on the Waymo validation set against another multi-task lidar only method.
Class-wise IoU was not available for LidarMultiNet for semantic segmentation on the validation set.}}
\label{tab:waymo-val-od-semseg}
\begin{tabular}{@{}c|ccc|cccccccccc@{}}
\toprule
 & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Object detection\\ mAPH - L2\end{tabular}} & \multicolumn{10}{c}{\begin{tabular}[c]{@{}c@{}}Semantic segmentation \\ class wise IoU and mIoU\end{tabular}} \\ \cmidrule(l){2-14} 
\multirow{-2}{*}{Method} & \cellcolor[HTML]{FFCCC9}\textit{Veh.} & \cellcolor[HTML]{F1B3F7}\textit{Ped.} & \cellcolor[HTML]{ECF4FF}\textit{Cyc.} & \cellcolor[HTML]{FFCCC9}\textit{Car} & \cellcolor[HTML]{FFCE93}\textit{Truck} & \cellcolor[HTML]{FFFC9E}\textit{Bus} & \cellcolor[HTML]{F1B3F7}\textit{Ped.} & \cellcolor[HTML]{ECF4FF}\textit{Bicyclist} & \cellcolor[HTML]{CBCEFB}\textit{Motorcyclist} & \cellcolor[HTML]{9AFF99}\textit{Veg.} & \cellcolor[HTML]{96FFFB}\textit{Building} & \cellcolor[HTML]{C0C0C0}\textit{Road} & \textbf{mIoU} \\ \midrule
LidarMultiNet\cite{ye2022lidarmultinet} & \textbf{73.38} & \textbf{74.10} & \textbf{77.96} & - & - & - & - & - & - & - & - & - & 72.40 \\
\cellcolor[HTML]{EFEFEF}\textbf{LiDAR-BEVMTN} & 72.70 & 69.42 & 71.10 & \cellcolor[HTML]{EFEFEF}89.77 & \cellcolor[HTML]{EFEFEF}60.92 & \cellcolor[HTML]{EFEFEF}65.12 & \cellcolor[HTML]{EFEFEF}60.64 & \cellcolor[HTML]{EFEFEF}61.32 & \cellcolor[HTML]{EFEFEF}61.01 & \cellcolor[HTML]{EFEFEF}88.63 & \cellcolor[HTML]{EFEFEF}80.13 & \cellcolor[HTML]{EFEFEF}93.10 & \cellcolor[HTML]{EFEFEF}\textbf{73.40} \\ \bottomrule
\end{tabular}
\end{table*}
\par








% --------------------------------------------------------------------------------------------------------- %
% \begin{table}[t]
% \centering
% \captionsetup{singlelinecheck=false, font=small, skip=2pt, belowskip=-2pt}
% \caption{\textbf{\textcolor{blue}{Timing analysis of each DB stage under different optimizations. Number of filters increase as 32-64-128-256-512 from DB1 to DB5 while spatial resolution of input is halved in each DB block.}}}
% \label{tab:timing_db}
% \scalebox{0.45}{
% \begin{adjustbox}{width=\columnwidth}
% % \setlength{\tabcolsep}{0.2em}
% \begin{tabular}{@{}cccc@{}}
% \toprule
% \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textit{\begin{tabular}[c]{@{}c@{}}DB\\ stage\end{tabular}}} & \cellcolor[HTML]{FFCCC9}\textit{pth} & \cellcolor[HTML]{FFFC9E}\textit{trt32} & \cellcolor[HTML]{9AFF99}\textit{trt16} \\ \midrule
% \multicolumn{1}{c|}{1} & 20.99 & 10.58 & 5.36 \\
% \multicolumn{1}{c|}{2} & 11.81 & 8.01 & 3.09 \\
% \multicolumn{1}{c|}{3} & 7.98 & 6.11 & 1.51 \\
% \multicolumn{1}{c|}{4} & 6.98 & 6.49 & 1.10 \\
% \multicolumn{1}{c|}{5} & 6.19 & 5.06 & 1.10 \\ \midrule
% Total & 53.95 & 36.25 & 11.86
% \end{tabular}
% \end{adjustbox}
% }
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}



% ----------- ORIGINAL: DO NOT DELETE -------------------%



% \begin{table}[t]
% \centering
% \captionsetup{singlelinecheck=false, font=small, skip=2pt, belowskip=-2pt}
% \caption{\textbf{Inference latency comparison}- \textcolor{blue}{MTL and STL} networks for Object Detection (OD), Semantic Segmentation (SS), and Motion Segmentation (MS).
% MTL - 3 tasks achieves 3x speed up over three single task networks.}
% \label{tab:table-latency-comparison}
% \begin{adjustbox}{width=0.9\columnwidth}
% \begin{tabular}{@{}l|c|c@{}}
% \toprule
% \multirow{2}{*}{\textit{Task combination}} &
%   \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}FP16 Inference\\ Latency (ms)\end{tabular}}} &
%   \multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Speedup \\ factor\end{tabular}}} \\
%                             &      &          \\ \midrule
% STL(OD) + STL(SS) + STL(MS) & 8.80 & baseline \\
% STL (OD) + MTL(SS + MS)     & 5.65 & 1.55     \\
% STL(MS) + MTL(OD + SS)      & 5.83 & 1.50     \\
% \rowcolor{gray9}MTL (OD + SS + MS)          & \textbf{3.01} & \textbf{2.92}     \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}

